Lattice Coding for Downlink Multiuser Transmission

In this thesis, we mainly investigate the lattice coding problem of the downlink communication between a base station and multiple users. The base station broadcasts a message containing each user's intended message. The capacity limit of such a system setting is already well-known while the design of practical coding and modulation schemes to approach the theoretical limit has not been fully studied and investigated in the literature. This thesis attempts to address this problem by providing a systematic design on lattice coding and modulation schemes for downlink multiuser communication systems. The main idea is to exploit the structure property of lattices to harness interference from downlink users.

==> Makefile <==
THESIS = thesis

TEXFILES = $(THESIS).tex mymacros.sty adfatitlepage.sty \
		misc/abstract.tex misc/ack.tex misc/library.tex \
		misc/declaration.tex  misc/pubs.tex misc/abbr.tex \
		chapter/intro.tex chapter/opt.tex \
		chapter/constr.tex chapter/manyobj.tex chapter/ccea.tex chapter/tdsa.tex \
		chapter/eng_problems.tex chapter/conclusion.tex \
		appendix/f-series.tex appendix/g-series.tex \
		appendix/cf.tex appendix/ctp.tex appendix/eng_prob.tex appendix/cf.tex  


all: $(THESIS).dvi
final: $(THESIS).ps $(THESIS).pdf

%.dvi: %.tex
	latex $<
	bibtex $(*F)
	bibtex bu1
	bibtex bu2
	bibtex bu3
	latex $<
	latex $<
	makeindex $(*F).nlo -s nomencl.ist -o $(*F).nls
	latex $<

%.bbl: %.tex
	latex $<
	bibtex $(*F)

%.ps: %.dvi
	dvips -Ppdf -G0 -ta4 -o $@ $<
	#dvips -Ppdf -o $@ $<

%.pdf: %.ps
	ps2pdf $< $@
	
$(THESIS).dvi: $(TEXFILES)

clean:
	rm -f *.aux chapter/*.aux misc/*.aux appendix/*.aux *.blg *.log *.bbl *.loa *.lof *.lot *.dvi *.nlo *.nls

realclean: clean
	rm -f *.ps *.pdf	

.PHONY: all final clean realclean

